Simulation-Free Hierarchical Latent Policy Planning for Proactive Dialogues

Recent advancements in proactive dialogues have garnered significant attention, particularly for more complex objectives (e.g. emotion support and persuasion). Unlike traditional task-oriented dialogues, proactive dialogues demand advanced policy planning and adaptability, requiring rich scenarios and comprehensive policy repositories to develop such systems. However, existing approaches tend to rely on Large Language Models (LLMs) for user simulation and online learning, leading to biases that diverge from realistic scenarios and result in suboptimal efficiency. Moreover, these methods depend on manually defined, context-independent, coarse-grained policies, which not only incur high expert costs but also raise concerns regarding their completeness. In our work, we highlight the potential for automatically discovering policies directly from raw, real-world dialogue records. To this end, we introduce a novel dialogue policy planning framework, LDPP. It fully automates the process from mining policies in dialogue records to learning policy planning. Specifically, we employ a variant of the Variational Autoencoder to discover fine-grained policies represented as latent vectors. After automatically annotating the data with these latent policy labels, we propose an Offline Hierarchical Reinforcement Learning (RL) algorithm in the latent space to develop effective policy planning capabilities. Our experiments demonstrate that LDPP outperforms existing methods on two proactive scenarios, even surpassing ChatGPT with only a 1.8-billion-parameter LLM.

==> Figures/illustration.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Images/demonstration2.pdf}
    \caption{An illustration of the proactive dialogue process and the hierarchical Markov Decision Process modeling in this work. This chat example is from ESConv~\cite{Liu2021TowardsES}.} 
    % \vspace{-0.2cm}
    \label{fig:illustration}
\end{figure}

==> Figures/visual_extes.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{Images/visual_extes2.pdf}
    \caption{Visualization of latent policies for utterances belonging to top-6 most frequently used policies on ExTES.} 
    % \vspace{-0.2cm}
    \label{fig:visual_extes}
\end{figure}

==> Figures/visual_p4g.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{Images/visual_p4g2.pdf}
    \caption{Visualization of latent policies for utterances corresponding to top-4 most frequently used policies on P4G.} 
    % \vspace{-0.2cm}
    \label{fig:visual_p4g}
\end{figure}

==> Sections/8-reproducibility_checklist.tex <==
\clearpage

\section{Reproducibility Checklist}
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes})
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{yes})
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{yes})
\end{itemize}


Does this paper make theoretical contributions? (\textbf{yes})

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (\textbf{yes})
    \item All novel claims are stated formally (e.g., in theorem statements). (\textbf{yes})
    \item Proofs of all novel claims are included. (\textbf{yes})
    \item Proof sketches or intuitions are given for complex and/or novel results. (\textbf{yes})
    \item Appropriate citations to theoretical tools used are given. (\textbf{yes})
    \item All theoretical claims are demonstrated empirically to hold. (\textbf{yes})
    \item All experimental code used to eliminate or disprove claims is included. (\textbf{yes})
\end{itemize}

Does this paper rely on one or more datasets? (\textbf{yes})

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\textbf{yes})
    \item All novel datasets introduced in this paper are included in a data appendix. (\textbf{yes})
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textbf{yes})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textbf{yes})
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\textbf{yes})
\end{itemize}


Does this paper include computational experiments? (\textbf{yes})

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (\textbf{yes, please see the supplementary materials.})
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{yes, please see the supplementary materials.})
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (\textbf{yes})
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{yes})
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{yes})
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes})
    \item This paper states the number of algorithm runs used to compute each reported result. (\textbf{no, we only run at least twice evaluations for main experiments in Table 1})
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{no, but we present the average performance for the main results in Table 1})
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\textbf{no})
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{partial, we list part of significant hyperpameters in appendix in Table 7 and 8})
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{partial, we only tried different values for significant hyperpameters ($T, L, K$) and present results in the parameter sensitivity analysis experiments})
\end{itemize}













==> Tables/human_eval_extes.tex <==
\begin{table}[!t]
    \centering
    % \subtable[ExTES]{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \textbf{LDPP} & \multicolumn{2}{c}{\textbf{Ide.}} & \multicolumn{2}{c}{\textbf{Com.}} & \multicolumn{2}{c}{\textbf{Sug.}} & \multicolumn{2}{c}{\textbf{Ove.}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
    vs. & Win & Lose & Win & Lose & Win & Lose & Win & Lose \\
    \midrule
    \textbf{PPDPP} & 8\% & 8\% & 52\% & 6\% & 64\% & 8\% & 68\% & 10\% \\
    \textbf{LoRA} & 6\% & 32\% & 6\% & 6\% & 32\% & 10\% & 26\% & 18\% \\
    \bottomrule
    \end{tabular}
    }
    % }
    % \subtable[P4G]{
    % \resizebox{0.85\linewidth}{!}{
    % \begin{tabular}{lcccccc}
    % \toprule
    % \textbf{LDPP} & \multicolumn{2}{c}{\textbf{Inf.}} & \multicolumn{2}{c}{\textbf{Per.}} & \multicolumn{2}{c}{\textbf{Ove.}} \\
    % \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    % vs. & Win & Lose & Win & Lose & Win & Lose \\
    % \midrule
    % \textbf{LoRA} &  &  &  &  &  &  \\
    % \textbf{PPDPP} &  &  &  &  &  &  \\
    % \bottomrule
    % \end{tabular}
    % }
    % }
    \caption{Human evaluation results on ExTES.}
    \label{tab:human_eval_extes}
\end{table}

==> Tables/human_eval_p4g.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{LDPP} & \multicolumn{2}{c}{\textbf{Inf.}} & \multicolumn{2}{c}{\textbf{Per.}} & \multicolumn{2}{c}{\textbf{Ove.}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    vs. & Win & Lose & Win & Lose & Win & Lose \\
    \midrule
    \textbf{PPDPP} & 32\% & 20\% & 40\% & 26\% & 48\% & 22\% \\
    \textbf{LoRA} & 10\% & 14\% & 24\% & 16\% & 26\% & 16\% \\
    \bottomrule
    \end{tabular}
    }
    \caption{Human evaluation results on P4G.}
    \label{tab:human_eval_p4g}
\end{table}

==> Tables/llm_base_size.tex <==
\begin{table}[t]
    \centering
    \renewcommand*{\arraystretch}{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{ExTES}} & \multicolumn{2}{c}{\textbf{P4G}}\\
    & AT$\downarrow$ & SR$\uparrow$ & AT$\downarrow$ & SR$\uparrow$\\
    \midrule
    \multicolumn{1}{l}{1.8b} &  &  &  &  \\
    \multicolumn{1}{l}{AnE~\cite{zhang2023ask}} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ ChatGPT} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ Qwen1.5-1.8b} &  &  &  &  \\
    % \multicolumn{1}{l}{Proactive~\cite{deng2023prompting}} &  &  &  &  \\
    % \multicolumn{1}{l}{$\quad$+ ChatGPT} &  &  &  &  \\
    % \multicolumn{1}{l}{$\quad$+ Qwen1.5-1.8b} &  &  &  &  \\
    \multicolumn{1}{l}{ProCoT~\cite{deng2023prompting}} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ ChatGPT} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ Qwen1.5-1.8b} &  &  &  &  \\
    \multicolumn{1}{l}{ICL-AIF~\cite{fu2023improving}} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ ChatGPT} &  &  &  &  \\
    \multicolumn{1}{l}{$\quad$+ Qwen1.5-1.8b} &  &  &  &  \\
    \midrule
    \multicolumn{1}{l}{Lora Fine-tuning} &  &  &  &  \\
    \midrule
    \multicolumn{1}{l}{LDPP} &  &  &  &  \\
    \bottomrule
    \end{tabular}
    }
    \caption{Main results on ExTES and P4G.}
    \label{tab:static_results}
\end{table}
